Decentralized Social Navigation with Non-Cooperative Robots via Bi-Level Optimization

This paper presents a fully decentralized approach for realtime non-cooperative multi-robot navigation in social mini-games, such as navigating through a narrow doorway or negotiating right of way at a corridor intersection. Our contribution is a new realtime bi-level optimization algorithm, in which the top-level optimization consists of computing a fair and collision-free ordering followed by the bottom-level optimization which plans optimal trajectories conditioned on the ordering. We show that, given such a priority order, we can impose simple kinodynamic constraints on each robot that are sufficient for it to plan collision-free trajectories with minimal deviation from their preferred velocities, similar to how humans navigate in these scenarios. We successfully deploy the proposed algorithm in the real world using F$1/10$ robots, a Clearpath Jackal, and a Boston Dynamics Spot as well as in simulation using the SocialGym 2.0 multi-agent social navigation simulator, in the doorway and corridor intersection scenarios. We compare with state-of-the-art social navigation methods using multi-agent reinforcement learning, collision avoidance algorithms, and crowd simulation models. We show that $(i)$ classical navigation performs $44\%$ better than the state-of-the-art learning-based social navigation algorithms, $(ii)$ without a scheduling protocol, our approach results in collisions in social mini-games $(iii)$ our approach yields $2\times$ and $5\times$ fewer velocity changes than CADRL in doorways and intersections, and finally $(iv)$ bi-level navigation in doorways at a flow rate of $2.8 - 3.3$ (ms)$^{-1}$ is comparable to flow rate in human navigation at a flow rate of $4$ (ms)$^{-1}$.

==> algorithms/kinodynamic.tex <==
\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
\SetKwComment{Comment}{$\triangleright$\ }{$40$Hz cycle frequency}
\SetAlgoLined
\Input{$\sigma_\textsc{opt} = \sigma^1\sigma^2 \ldots \sigma_{\lvert \mathcal{C}^t_{\mathcal{O}} \rvert}$}
\Output{$\Xi^i_{\sigma_i}$}

\uIf{$\sigma^i = 1$}{
$v_\textrm{max}$ = \texttt{V\_MAX}
}
\Else{$v_\textrm{max}=$ \texttt{V\_MAX}/$\sigma^i$}

\caption{Retrieving kinodynamic constraints}
\label{algo: kino}
% \vspace{-10pt}
\end{algorithm}

==> algorithms/overall.tex <==
\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
\SetKwComment{Comment}{$\triangleright$\ }{}
\SetAlgoLined
\Input{Map $m$, initial pose, and goals}
\Output{$v, \omega$}
A$^*$ path $\gets$ \textsc{Get Global Path}\\
$v, \omega \gets$ \textsc{Local Planning}(A$^*$ path, $o^i_t, \Xi$)\\

\caption{Overview of the navigation system}
\label{algo: overall}
% \vspace{-10pt}
\end{algorithm}

==> sections/theory.tex <==
\section{Proof}

\subsection{Proving convergence}

\subsection{Safety guarantees}
